The dependence of protostar formation on the geometry and strength of the initial magnetic field

We report results from twelve simulations of the collapse of a molecular cloud core to form one or more protostars, comprising three field strengths (mass-to-flux ratios, {\mu}, of 5, 10, and 20) and four field geometries (with values of the angle between the field and rotation axes, {\theta}, of 0{\deg}, 20{\deg}, 45{\deg}, and 90{\deg}), using a smoothed particle magnetohydrodynamics method. We find that the values of both parameters have a strong effect on the resultant protostellar system and outflows. This ranges from the formation of binary systems when {\mu} = 20 to strikingly differing outflow structures for differing values of {\theta}, in particular highly suppressed outflows when {\theta} = 90{\deg}. Misaligned magnetic fields can also produce warped pseudo-discs where the outer regions align perpendicular to the magnetic field but the innermost region re-orientates to be perpendicular to the rotation axis. We follow the collapse to sizes comparable to those of first cores and find that none of the outflow speeds exceed 8 km s$^{-1}$. These results may place constraints on both observed protostellar outflows, and also on which molecular cloud cores may eventually form either single stars and binaries: a sufficiently weak magnetic field may allow for disc fragmentation, whilst conversely the greater angular momentum transport of a strong field may inhibit disc fragmentation.

==> macros.tex <==
%!TEX root=./thesis.tex
%%% My macros
% Helper
\newcommand*{\unitsep}{\ensuremath{\cdot}}
\makeatletter
\@ifclassloaded{mnras}{\renewcommand*{\unitsep}{\thinspace}}% For MNRAS
\makeatother
% Operators
\newcommand*{\Dt}{\ensuremath{\mathrm{D}_t}\xspace}
\newcommand*{\Laplace}{\mathop{}\!\mathbin\bigtriangleup} % Yeah I don't understand this either
% Maths punctuation
\newcommand*{\comma}{\ensuremath{\text{,}}\xspace}
\newcommand*{\fstop}{\ensuremath{\text{.}}\xspace}
% Units (simple)
\newcommand*{\au}{\ensuremath{\text{au}}\xspace}
\newcommand*{\kelvin}{\ensuremath{\text{K}}\xspace}
\newcommand*{\cm}{\ensuremath{\text{cm}}\xspace}
\newcommand*{\km}{\ensuremath{\text{km}}\xspace}
\newcommand*{\gram}{\ensuremath{\text{g}}\xspace}
\newcommand*{\second}{\ensuremath{\text{s}}\xspace}
\newcommand*{\solarm}{\ensuremath{\text{M}_\odot}\xspace}
%\newcommand*{\yr}{\ensuremath{\text{a}}\xspace}
\newcommand*{\uyear}{a}
\makeatletter
\@ifclassloaded{mnras}{\renewcommand*{\uyear}{yr}}% For MNRAS
\makeatother
\newcommand*{\yr}{\ensuremath{\text{\uyear}}\xspace}%MNRAS use yr :-@
\newcommand*{\rad}{\ensuremath{\text{rad}}\xspace}
\newcommand*{\gauss}{\ensuremath{\text{G}}\xspace}
% Units (composite)
\newcommand*{\dens}{\gram\unitsep\cm^{-3}\xspace}
\newcommand*{\velo}{\cm\unitsep\second^{-1}\xspace}
\newcommand*{\kvelo}{\km\unitsep\second^{-1}\xspace}
\newcommand*{\rads}{\rad\unitsep\second^{-1}\xspace}
\newcommand*{\mugauss}{~\micromu\gauss\xspace} % nbspace before, nothing in between.
% Units (other)
\newcommand*{\micromu}{\ensuremath{\text{\textgreek{μ}}}} %Yuk! Necessary to get the `right' upright greek. NOTE: no \xspace here -- it's still wrong, but only a thin space wrong
\newcommand*{\tff}{\ensuremath{t_\rmn{ff}}\xspace}
\newcommand*{\Henry}{\ensuremath{\text{H}}\xspace}
\newcommand*{\permeter}{\ensuremath{\text{m}^{-1}}\xspace}
\newcommand*{\dyne}{\ensuremath{\text{dyn}}\xspace}
\newcommand*{\erg}{\ensuremath{\text{erg}}\xspace}
\newcommand*{\parsec}{\ensuremath{\text{pc}}\xspace}

% Latin stuff
\let\latshape\itshape\xspace%Default
%\newcommand*{\latshape}{\itshape\xspace}
\makeatletter
\@ifclassloaded{mnras}{\renewcommand*{\latshape}{}}% For MNRAS
\makeatother
\newcommand*{\eg}{{\latshape e.g.}\xspace}
\newcommand*{\etc}{{\latshape etc.}\xspace}
\newcommand*{\ie}{{\latshape i.e.}\xspace}
\newcommand*{\etal}{{\latshape et al.}\xspace}
\newcommand*{\ia}{{\latshape inter alia}\xspace}
\newcommand*{\viz}{{\latshape viz.}\xspace}
\newcommand*{\ca}{{\latshape ca.}\xspace}
\newcommand*{\cf}{{\latshape cf.}\xspace}

% Text abbreviations - English
\newcommand*{\fst}{\textsu{st}\xspace}
\newcommand*{\scnd}{\textsu{nd}\xspace}
\newcommand*{\nth}{\textsu{th}\xspace}

% The ampersand
\newcommand*{\ampersand}{\textit{\&}\xspace}

% Other stuff
\makeatletter
%\@ifclassloaded{mnras}{% Provided by mnras.cls
\@ifundefined{arcsec}{\newcommand*{\arcsec}{\mbox{\ensuremath{^{\prime\prime}}}}}%  % arcsecond symbol: 0''
\@ifundefined{arcmin}{\newcommand*{\arcmin}{\mbox{\ensuremath{^{\prime}}}}}%  % arcsecond symbol: 0''
%}
\makeatother
\newcommand*{\HII}{\mbox{H\,{\footnotesize II}}}       % HII properly spaced
\newcommand*{\versesep}{\ensuremath{\cdot\quad\cdot\quad\cdot}}

% The Lagrangian
\newcommand*{\Lagr}{\ensuremath{\mathcal{L}}\xspace}
\newcommand*{\Kinet}{\ensuremath{\mathcal{T}}\xspace}
\newcommand*{\Poten}{\ensuremath{\mathcal{V}}\xspace}
\newcommand*{\Hamil}{\ensuremath{\mathcal{H}}\xspace}

\newcommand*{\eqdef}{\stackrel{\text{def}}{=}}

% Fields
\newcommand*{\scalarfield}[2][]{\ensuremath{#2_{#1}}}
\newcommand*{\vectorfield}[3][]{\ensuremath{#3^{#2}_{#1}}}
%\newcommand*{\scalarfield}[2][]{\ensuremath{#2\indices*{_{#1}}}}
%\newcommand*{\vectorfield}[3][]{\ensuremath{#3\indices*{^{#2}_{#1}}}}
\newcommand*{\dfield}[1][]{\scalarfield[#1]{\rho}}
\newcommand*{\gfield}[1][]{\scalarfield[#1]{\phi}}
\newcommand*{\pfield}[1][]{\scalarfield[#1]{p}} % We need to decide what to do about p_hyd.
\newcommand*{\radefield}[1][]{\scalarfield[#1]{\mathscr{E}}}
\newcommand*{\vfield}[2][]{\vectorfield[#1]{#2}{v}}
\newcommand*{\bfield}[2][]{\vectorfield[#1]{#2}{B}}
\newcommand*{\ffield}[2][]{\vectorfield[#1]{#2}{\mathscr{F}}}
% Tensors
\newcommand*{\tensorfield}[4][]{\ensuremath{#4^{#2 #3}_{#1}}}
%\newcommand*{\tensorfield}[4][]{\ensuremath{#4\indices*{^{#2 #3}_{#1}}}}
\newcommand*{\maxwell}[3][]{\tensorfield[#1]{#2}{#3}{\sigma}}
\newcommand*{\radpressure}[3][]{\tensorfield[#1]{#2}{#3}{P}}

% Odds and ends
\newcommand*{\nabl}[2][]{\vectorfield[#1]{#2}{\nabla}}
\newcommand*{\kronecker}[2]{\tensorfield{#1}{#2}{\delta}}
\newcommand*{\tensorfieldthree}[5][]{\ensuremath{#5^{#2 #3 #4}_{#1}}}
\newcommand*{\levicivita}[3]{\tensorfieldthree{#1}{#2}{#3}{\epsilon}}

% The Kernel
\newcommand*{\kernel}[1]{W_{ab}\left(h_{#1}\right)}

% Lazy typist/sorthands/etc.
\makeatletter\@ifundefined{rmn}{\def\rmn{\mathrm}}\makeatother % Older mnras.cls provides this.
\def\udens{\dens} % Too lazy to fix typos...
% Textual
\newcommand*{\fnm}{\footnotemark\xspace}
\newcommand*{\sphng}{\texttt{sphNG}\xspace}
\newcommand*{\ndspmhd}{\texttt{ndspmhd}\xspace}
\newcommand*{\phantomcode}{\texttt{Phantom}\xspace}
\newcommand*{\openmp}{\texttt{openMP}\xspace}
\newcommand*{\mpi}{\texttt{MPI}\xspace}
\newcommand*{\privcom}{\textit{priv. comm.}\xspace}
\newcommand*{\privcomb}{(\privcom)\xspace}
\newcommand*{\submitted}{\textit{subm.}\xspace}
\newcommand*{\submittedb}{(\submitted)\xspace}
\newcommand*{\inprep}{\textit{in prep.}\xspace}
\newcommand*{\inprepb}{(\submitted)\xspace}
% Mathsey
\newcommand*{\betaplasma}{\ensuremath{\beta_\mathrm{plasma}}\xspace}

\newcommand*{\abbrsep}{.}
\newcommand*{\SPH}{S\abbrsep{}P\abbrsep{}H\abbrsep{}\xspace}
\newcommand*{\SPMHD}{S\abbrsep{}P\abbrsep{}M\abbrsep{}H\abbrsep{}D\abbrsep{}\xspace}
\newcommand*{\SPRHD}{S\abbrsep{}P\abbrsep{}R\abbrsep{}H\abbrsep{}D\abbrsep{}\xspace}
\newcommand*{\MHD}{M\abbrsep{}H\abbrsep{}D\abbrsep{}\xspace}
\newcommand*{\RHD}{R\abbrsep{}H\abbrsep{}D\abbrsep{}\xspace}
\newcommand*{\FLD}{F\abbrsep{}L\abbrsep{}D\abbrsep{}\xspace}
\newcommand*{\RT}{R\abbrsep{}T\abbrsep{}\xspace}
\newcommand*{\SN}{S\abbrsep{}N\abbrsep{}\xspace}

\newcommand*{\marith}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand*{\garith}{\ensuremath{\mathfrak{G}}\xspace}
\newcommand*{\harith}{\ensuremath{\mathfrak{H}}\xspace}
\newcommand*{\qarith}{\ensuremath{\mathfrak{Q}}\xspace}
